Multicarrier PAPR Reduction by Iteratively Shifting and Concentrating the Probability Measure

The peak power problem in multicarrier waveforms is well-known and imposes substantial limitations on wireless communications. As the quest for investigation of enabling technologies for the next generation of wireless communication systems 5G is at its peak, the problem is re-emerging in a much broader range of technologies. However, despite numerous publications on the topic, there is no well-established structure available for the problem, which motivates a boost in research. In this paper, a novel peak power reduction algorithm is proposed which offers a substantial Peak-to-Average Power Ratio (PAPR) reduction and exhibits high potential for further refinements. Mathematical tractability of the algorithm is expected to be of particular importance to this end. A remarkable early observation is a PAPR reduction of about 4.5 dB for 64 subcarriers with a rate loss of 0.5 bits per complex data symbol in an OFDM scheme, which is half the rate loss that other methods require in this class of algorithms.

==> tikz-files/frame-double.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (13.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\foreach \x in {3,4,5}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\foreach \x in {6,7,8}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (9,1) rectangle +(0.5,-0.15);


\foreach \x in {6,7,8}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);

\foreach \x in {9,10,11}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);


\fill [draw=blue, fill=white, rounded corners=0.02cm] (12,1.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/frame-single.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (7.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \xone/\y in {0/0.8, 0.5/1, 1/1.3, 1.5/1.5, 2/1.8, 2.5/2}
{
	\draw [blue,|-|] (\xone,\y) -- +(4,0);
}

\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/pts-oqam-structure.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\usetikzlibrary{positioning}
%
%\input{ tikz-styles}
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}

%%%%%%%%the modulator

\node[block,minimum width=1.5cm] (filter1) {SFB};
\node[block,minimum width=1.5cm] (filter2) [below=of filter1, yshift=0.5cm] {SFB};
\node[block,minimum width=1.5cm] (filter3) [below=of filter2, yshift=0.5cm] {SFB};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (partitioning) [left of=filter1, xshift=-0.2cm, yshift=+2cm] {Partitioning};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (OQAMpre) [left of=filter1, xshift=-0.2cm, yshift=+3.8cm] {OQAM pre-preprocessing};

\node[block,minimum width=1cm, minimum height=3.7cm] (sum) [right of=filter2, xshift=4cm, yshift=0cm] {$\sum$};


\node (mul1) [summul, right of=filter1, xshift=1cm] {$\times$};
\node (mul2) [summul, right of=filter2, xshift=1.5cm] {$\times$};
\node (mul3) [summul, right of=filter3, xshift=2cm] {$\times$};

\draw [<-] (mul1) -- +(0,0.6cm) node [anchor=west]{$p_1$};
\draw [<-] (mul2) -- +(0,0.6cm) node [anchor=west]{$p_2$};
\draw [<-] (mul3) -- +(0,0.6cm) node [anchor=west]{$p_3$};

\foreach \x in {1,2,3}
	\draw [->] (filter\x) -- (mul\x);

\draw [->] (mul1.east) -- +(2.32cm,0);
\draw [->] (mul2.east) -- +(1.82cm,0);
\draw [->] (mul3.east) -- +(1.32cm,0);

\node[block,minimum width=2.4cm, minimum height=1cm] (opt) [below of=mul2, xshift=0cm, yshift=-2cm] {Optimization};

\draw [<-] (mul1) |- (opt.north);
\draw [<-] (mul2) -- (opt);
\draw [<-] (mul3) |- (opt.north);
%\draw [<-] (mul2) -- +(0cm,0);
%\draw [<-] (mul3) -- +(0cm,0);

%\foreach \x/\n in {1/0,2/1,3/N-1}
%	\draw [<-] (mul\x) -- +(0,0.5cm) node [anchor=south] {$\beta_{\n}$};

\foreach \x in {1,2,3}
{
	\draw [<-] (filter\x.west) -- +(-0.73cm,0) ;		%between SFB and partitioning
}

\draw [->] (filter1.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,0}$};  %between input and OQAM
\draw [->] (filter2.west) +(-4.5cm,0.5cm)-- +(-3.55cm,0.5cm) node [anchor=south east] {$A_{k,1}$};  %between input and OQAM
\draw [->] (filter3.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,N-1}$};  %between input and OQAM

\draw [->] (filter1.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	
\draw [->] (filter2.west) +(-2.55cm,0.5cm)-- +(-1.75cm,0.5cm) ;	%between OQAM and partitioning	
\draw [->] (filter3.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	

\node[circle, fill=black, left=of partitioning, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.3cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[circle, fill=black, left=of OQAMpre, yshift=1.9cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[block,minimum width=2cm, minimum height=1cm] (buffer) [above of=sum, xshift=-0.5cm, yshift=1.7cm] {Buffer};

\draw [->] (buffer.west) -- +(-0.3cm,0) -- +(-0.3cm,-1.2cm) -- +(1cm,-1.2cm);
\draw [->] (sum.east) +(1cm,0) |- (opt.east);
\draw [->] (sum.east) +(1cm,0) |- (buffer.east);
\draw [->] (sum.east) -- +(1.5cm,0) node [anchor=south] {$s[k]$};


	
\end{tikzpicture}
%\end{figure}
%\end{document}

